TSN-Affinity: Similarity-Driven Parameter Reuse for Continual Offline Reinforcement Learning

Continual offline reinforcement learning (CORL) aims to learn a sequence of tasks from datasets collected over time while preserving performance on previously learned tasks. This setting corresponds to domains where new tasks arise over time, but adapting the model in live environment interactions is expensive, risky, or impossible. However, CORL inherits the dual difficulty of offline reinforcement learning and adapting while preventing catastrophic forgetting. Replay-based continual learning approaches remain a strong baseline but incur memory overhead and suffer from a distribution mismatch between replayed samples and newly learned policies. At the same time, architectural continual learning methods have shown strong potential in supervised learning but remain underexplored in CORL. In this work, we propose TSN-Affinity, a novel CORL method based on TinySubNetworks and Decision Transformer. The method enables task-specific parameterization and controlled knowledge sharing through a RL-aware reuse strategy that routes tasks according to action compatibility and latent similarity. We evaluate the approach on benchmarks based on Atari games and simulations of manipulation tasks with the Franka Emika Panda robotic arm, covering both discrete and continuous control. Results show strong retention from sparse SubNetworks, with routing further improving multi-task performance. Our findings suggest that similarity-guided architectural reuse is a strong and viable alternative to replay-based strategies in a CORL setting. Our code is available at: https://github.com/anonymized-for-submission123/tsn-affinity.

==> figures/tsn-affinite.tex <==
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tikzpicture}[
    x=1cm,
    y=1cm,
    >=Latex,
    font=\small,
    panel/.style={
        draw=none,
        rounded corners=3pt
    },
    copybox/.style={
        draw,
        rounded corners=4pt,
        line width=0.9pt,
        fill=gray!10
    },
    smalltask/.style={
        draw,
        rounded corners=2pt,
        line width=0.8pt,
        fill=white,
        minimum width=1.1cm,
        minimum height=0.65cm,
        font=\normalsize
    },
    mainbox/.style={
        draw,
        rounded corners=2.5pt,
        line width=0.8pt,
        fill=white,
        minimum width=2.1cm,
        minimum height=0.9cm,
        align=center
    },
    decision/.style={
        diamond,
        draw,
        aspect=1.8,
        line width=0.8pt,
        fill=white,
        align=center,
        inner sep=1.5pt
    },
    trainbox/.style={
        draw,
        rounded corners=4pt,
        line width=1.0pt,
        fill=green!8
    },
    spawnbox/.style={
        draw,
        rounded corners=4pt,
        line width=0.9pt,
        fill=gray!8
    },
    arr/.style={->, line width=0.85pt},
    dashedarr/.style={->, dashed, line width=0.9pt, orange!85!black},
    faint/.style={line width=0.8pt, gray!50},
    reused/.style={line width=1.2pt, red!75},
    neww/.style={line width=1.2pt, dashed, orange!85!black},
    inactive/.style={line width=1.0pt, gray!55},
]

% =========================================================
% TITLES
% =========================================================
\node[font=\bfseries\Large] at (4.7,9.3) {Incoming};
\node[font=\bfseries\Large] at (4.7,8.8) {Task};

\node[font=\bfseries\Large] at (11.1,8.5) {Training};

% =========================================================
% LEFT PANEL: COPIES
% =========================================================
\node[font=\bfseries\large] at (1.7,7.65) {Copy 1};

\draw[copybox] (0.2,4.7) rectangle (3.2,7.3);

% task labels in copy 1
\node[smalltask] at (1.1,6.75) {$\mathcal{T}_1$};
\node[smalltask] at (2.35,6.75) {$\mathcal{T}_2$};

% subnet for T1
\fill[blue!70] (0.78,5.65) circle (0.05);
\fill[blue!70] (1.18,5.30) circle (0.05);
\fill[blue!70] (1.58,5.65) circle (0.05);
\draw[blue!70, line width=1.0pt] (0.78,5.65) -- (1.18,5.30) -- (1.58,5.65);

% subnet for T2
\fill[red!75] (2.02,5.25) circle (0.05);
\fill[red!75] (2.40,5.62) circle (0.05);
\fill[red!75] (2.78,5.25) circle (0.05);
\draw[red!75, line width=1.0pt] (2.02,5.25) -- (2.40,5.62) -- (2.78,5.25);

% Copy 2
\node[font=\bfseries\large] at (1.7,4.15) {Copy 2};

\draw[copybox] (0.2,1.35) rectangle (3.2,3.95);

\node[smalltask] at (1.7,3.35) {$\mathcal{T}_3$};

\fill[teal!70!black] (0.95,2.10) circle (0.05);
\fill[teal!70!black] (1.35,2.45) circle (0.05);
\fill[teal!70!black] (1.75,2.10) circle (0.05);
\fill[teal!70!black] (2.15,2.45) circle (0.05);
\draw[teal!70!black, line width=1.0pt] (0.95,2.10) -- (1.35,2.45) -- (1.75,2.10) -- (2.15,2.45);

\node[align=center, font=\Large] at (1.7,0.45) {task-specific masks stored\\within multiple model copies};

% dashed orange reference arrow from copy 1 to routing
\draw[dashedarr] (3.2,6.15) -- (4.15,6.5);

% =========================================================
% MIDDLE PANEL: ROUTING
% =========================================================
% incoming task box
\draw[mainbox, minimum width=1.7cm, minimum height=0.9cm] (4.0,7.85) rectangle (5.7,8.75);
\node at (4.85,8.30) {$T\_4$};

% line downward from incoming task
\draw[arr] (4.85,7.85) -- (4.85,7.25);

% action and latent affinity
\node[mainbox, minimum width=1.8cm] (action) at (3.85,6.45) {Action Affinity};
\node[mainbox, minimum width=1.8cm] (latent) at (5.85,6.45) {Latent Affinity};

\draw[arr] (4.85,7.25) -| (action.north);
\draw[arr] (4.85,7.25) -| (latent.north);

% routing score
\node[mainbox, minimum width=1.8cm] (score) at (4.85,5.15) {Routing score};

\draw[arr] (action.south) |- (score.north);
\draw[arr] (latent.south) |- (score.north);

% routing decision
\node[decision, minimum width=1.25cm, minimum height=1.0cm] (decision1) at (4.85,3.95) {Routing\\Decision};

\draw[arr] (score.south) -- (decision1.north);

% best source task

\node[
    mainbox,
    minimum width=1.2cm,
    minimum height=1.2cm,
    align=center
] (bestsrc) at (4.85,2.75) {$\mathcal{T}_j$\\best source\\task};

\draw[arr] (decision1.south) -- (bestsrc.north);

% should create new copy?
\node[decision, minimum width=1.45cm, minimum height=1.05cm] (decision2) at (4.85,1.55) {should create\\new copy?};

\draw[arr] (bestsrc.south) -- (decision2.north);

% route to right panels
\draw[arr] (decision1.east) -- ++(0.55,0) |- (8.95,4.75);
\draw[arr] (decision2.east) -- ++(1.8,0) |- (8.95,5.0);

% =========================================================
% RIGHT PANEL: TRAINING
% =========================================================
\node[font=\bfseries\large] at (10.8,7.35) {reuse selected copy};

\draw[trainbox] (8.7,4.7) rectangle (12.7,7.0);

% reused/protected graph inside
\fill[red!75] (9.45,6.28) circle (0.05);
\fill[red!75] (10.25,5.82) circle (0.05);
\fill[red!75] (11.25,6.22) circle (0.05);
\fill[red!75] (9.60,5.28) circle (0.05);
\fill[red!75] (10.55,4.95) circle (0.05);

\draw[reused] (9.45,6.28) -- (10.25,5.82) -- (11.25,6.22);
\draw[reused] (10.25,5.82) -- (9.60,5.28);
\draw[reused] (9.60,5.28) -- (10.55,4.95);

% new/trainable edges
\fill[orange!85!black] (11.75,5.72) circle (0.05);
\fill[orange!85!black] (11.32,4.92) circle (0.05);

\draw[neww] (10.25,5.82) -- (11.75,5.72);
\draw[neww] (10.25,5.82) -- (11.32,4.92);
\draw[neww] (10.55,4.95) -- (11.32,4.92);

% right text inside reuse box
\node[anchor=west, align=left] at (11.55,6.18) {frozen reused weights};
\node[anchor=west, align=left] at (11.55,5.55) {new sparse weights};

% legend
\draw[reused] (9.0,4.32) -- (9.7,4.32);
\node[anchor=west] at (9.95,4.32) {reused / protected};

\draw[neww] (9.0,3.98) -- (9.7,3.98);
\node[anchor=west] at (9.95,3.98) {new / trainable};

\draw[inactive] (9.0,3.64) -- (9.7,3.64);
\node[anchor=west] at (9.95,3.64) {inactive};

% spawn new copy
\draw[spawnbox] (9.0,1.2) rectangle (12.7,2.5);
\node[font=\large] at (10.85,1.85) {spawn new copy};

% faint incoming arrows from left of right panel
\fill[black] (8.72,5.75) -- (8.45,5.88) -- (8.45,5.62) -- cycle;
\fill[gray!55] (8.98,2.05) -- (8.71,2.18) -- (8.71,1.92) -- cycle;

\end{tikzpicture}
}
\caption{Overview of TSN-Affinity. Previously learned tasks are represented by sparse task-specific subnetworks. Given a new task $\mathcal{T}_t$, the method computes an affinity score with respect to prior tasks and routes the new task to the most related subnetwork. Parameters in the selected subnetwork are reused in a frozen form, while additional sparse capacity can be allocated for the new task, enabling transfer without destructive interference.}
\label{fig:tsn_affinity_clean}
\end{figure*}
